Study and evaluation of an Irregular Graph Algorithm on Multicore and GPU Processor Architectures

One area of Computing applications which poses significant challenge of performance scalability on Chip Multiprocessors(CMP's) are Irregular applications. Such applications have very little computation and unpredictable memory access patterns making them memory-bound in contrast to compute-bound applications. Since the gap between processor and memory performance continues to exist, difficulty to hide and decrease this gap is one of the important factors which results in poor performance of these applications on CMP's. The goal of this thesis is to overcome many such challenges posed during performance acceleration of an irregular graph algorithm called Triad Census. We accelerated the Triad Census algorithm on two significantly different Chip Multiprocessors: Dual-socket Intel Xeon Multicore (8 hardware threads per socket) and 240-processor core NVIDIA Tesla C1060 GPGPU(128 hardware threads per core). The experimental results obtained on Intel Multicore Xeon system shows performance speedups (w.r.t baseline sequential) of maximum 56x , average 33x and minimum 8.3x for real world graph data sets. On NVIDIA Tesla C1060 GPGPU, we were able to match almost equally the Multicore results - 58.4x maximum, 32.8x average and 4.2x minimum speedups w.r.t baseline sequential. In terms of raw performance, for the graph data set called Patents network, our results on Intel Xeon Multicore(16 hw threads) were 1.27x times faster than previous results on Cray XMT(16 hw threads) while results achieved on GPGPU were comparatively slower(0.72x). To the best of our knowledge, this algorithm has only been accelerated on supercomputer class computer named Cray XMT and no work exists that demonstrates performance evaluation and comparison of this algorithm on relatively lower-cost Multicore and GPGPU based platforms.

==> chapter-2/snatriad.tex <==
\chapter{Social Network Analysis and Triad Census Algorithm}
\label{chap:snatriad}
This chapter is about state of the art literature on Social Network Analysis (SNA) which forms the basis to understand the irregular Triad Census sparse graph algorithm. We also explain the working of the Triad census algorithm and some approaches used in literature for its parallelization on multiprocessor architectures.

\section{Social Network Analysis(SNA)}
\label{sec:sna}
\emph{Social network analysis or SNA}  deals with analysis of social network structures. It focuses on social entities and ties or relationship between them. Relationship could be friendship, beliefs, common interest, economic interactions etc. Examples of social structures are communities, market, societies, and countries. In SNA vocabulary, any entity involved in a social network is called an \emph{Actor}. An actor can refer to a person, organization, nation etc. basically any entity that can be conceptualized as an object with behavior and which can interact with other objects.
\\
\\
SNA involves conceptualizing, modeling, representing, visualizing such social structures and then detecting and interpreting patterns of social ties among the actors. It also deals with measurement of characteristics or metrics of social networks. Examples of such metrics are centrality (which actors are best connected to others, or have the most influence) in particular betweenness centrality of a vertex v(the number of shortest paths between all pairs of vertices in the network going through v), connectivity(how actors are related to one another), cohesion(how strong is the relationship between connected group of actors), transitivity(Is enemy of your friend is also your enemy?), clustering(are two neighbors of a vertex are also neighbors themselves), prestige, trust etc.

Social network analysis has also been linked with biology, communication studies, organizational studies, internet social networks, sociology, geography, finance and terrorism studies (Figure~\ref{fig:sna-examples}). As a result new forms of network analysis have emerged. For example SNA is used in epidemiology to help understand how patterns of human contact aid or inhibit the spread of diseases in a population such as HIV\protect\footnote{\href{http://www.respondentdrivensampling.org/reports/sociological_focus.pdf}{http://www.respondentdrivensampling.org/reports/sociological\_focus.pdf}} and obesity.

\begin{figure}
	\subfloat[][]
	{
	    \label{fig:sna-ex-1}
	    \includegraphics[angle=90, scale=1.5]{chapter-2/images/prof-net-new}
	 }	
	\subfloat[][]
	{
	    \label{fig:sna-ex-2}
	    \includegraphics[scale=0.4]{chapter-2/images/football-smaller-new}
	}
	\\
	\subfloat[][]
	{
	    \label{fig:sna-ex-3}
	    \includegraphics[scale=0.5]{chapter-2/images/human-protein-nw}
	}
	\subfloat[][]
	 {
	    \label{fig:sna-ex-4}
	    \includegraphics[scale=1]{chapter-2/images/soc-livejournal}
	 }

	\caption[]
	{ Examples of various social networks:
	    \subref{fig:sna-ex-1} My linkedin professional network
	    \subref{fig:sna-ex-2} Soccer pass network
	    \subref{fig:sna-ex-3} Human protein network
	    \subref{fig:sna-ex-4} Livejournal social network
	    \label{fig:sna-examples}
	}
\end{figure}

Graphs abstractions from graph theory provide an intuitive way of representing such social networks and applying various algorithms to capture social network metrics. Actors are represented as \emph{vertices} and relations between them are represented as \emph{edges} or \emph{arcs}. To make networks out of these graph representations, all real world information associated with actors and ties are associated with the vertices and edges of graph. For example consider a social graph of a soccer team\footnote{http://scientometrics.wordpress.com/} during a match (Figure~\ref{fig:sna-examples}), with vertices representing soccer players and arcs representing a pass from one player to another. By associating information such as player names with vertices and number of passes made between two players with thickness of the arc, one can make a social network out of it. This network can be analyzed for various metrics like which players made or received the most passes, percentage of passes made or received by defenders, which sequence of passes had a higher probability of scoring a goal, etc. Many tools  are available for analysis and visualization of such social networks namely Pajek, GUESS, ORA, and Cytoscape, NetworkX, SNAP, igraph.
\\
\\
Most of the real-world graph data sets are scale-free networks which exhibit power law degree distribution. Further many such networks in addition have characteristics of small-world network and can range from several hundreds to million and even billions of vertices and arcs/edges. What it means that most graph algorithms thus have to process such large-scale sparse graphs. The challenges therefore lies in compact space efficient and cache friendly  representations of such sparse graphs and then optimizing the graph algorithms for scalable parallel implementation on pervasive UMA and NUMA shared memory space chip-multiprocessors.

\section{Triad census algorithm}
\label{sec:triad-algo}
\emph{Triad census} based analysis are statistical methods that study and examine characteristics of social networks by studying properties of local 3-vertex-subgraphs present in a graph. The description of \emph{triad} and \emph{dyad} census in SNA was first studied and proposed by \citep*{Holland1970}. They introduced the concept of \emph{dyad and triad census} - number of 2-subgraphs and 3-subgraphs in a graph and also generic \emph{k-subgraph} census. \citep*{Wasserman1975} studied triad census for various random graph distributions. 
\\
\begin{figure}
	\centering
	\includegraphics[scale=0.8]{chapter-2/images/dyad-types}
	\caption{Dyad types}\label{fig:dyadtypes}
\end{figure}
\\
A \emph{triad} is defined as a digraph with 3 vertices and zero or more arcs connecting them. Similar to triad, a \emph{dyad} is a pair of vertices which have zero or more arcs between them. There can be four types of dyads(Figure ~\ref{fig:dyadtypes}): 1 - \emph{null dyad}, 2 - \emph{asymmetric dyads} and 1 - \emph{mutual dyad}. Only null dyad is a \emph{disconnected dyad}, other dyad types are \emph{connected dyads}. One can think of a triad to be made up of three dyads and therefore 64-possible triads(4*4*4, as each pair of vertices can be one of four possible dyads) can be formed from a \emph{strict digraph}(no loops) of order three. Further, these 64 triads can be merged into 16-unique \emph{isomorphic triads}. All triads can be classified into three triad classes namely \emph{null, dyadic and connected triads}
\\
\begin{figure}
    \centering
    \includegraphics[scale=0.6]{chapter-2/images/triad-types}
    \caption{Types of Triads}\label{fig:triadtypes}
\end{figure}

Figure~\ref{fig:triadtypes} shows the isomorphic types of triads numbered 1 to 16 and classification of these triads. Established convention of naming the 16 triad types uses a 3-digit code suffixed with an optional triad property: \(\mathsf{MAN<P>}\), where \(\mathsf{M}\) is number of \emph{mutual dyads}, \(\mathsf{A}\) is number of \emph{asymmetric dyads}, \(\mathsf{N}\) is the number of \emph{null dyads}, \(\mathsf{P}\) is an optional triad property. 
\\
\\
Each of the digits \(\mathsf{M, A, N}\) can range from 0 to 3. \(\mathsf{P}\) can take values U-up, C-cyclic, D-down, and T-transitive. So triad types 1-16 are classified and named as follows:

\begin{itemize}
\item \emph{Null triads}: 1- 003 
\item \emph{Dyadic triads}:  2 - 012, 3 - 102
\item \emph{Connected or complete triads}: 4 - 021D, 5 - 021U, 6 - 021C, 7- 111D, 8 - 111U, 9 - 030T, 10 - 030C, 11 - 201, 12 - 120D, 13 - 120U, 14 - 120C, 15 - 210, 16 - 300
\end{itemize}

Only null and dyadic triads are disconnected, all other triads are connected. \emph{Triad census algorithm} is a combinatorial problem that aims to count number of each of these 16 unique isomorphic or 64 triads in a given graph i.e. census of triads. By finding out frequencies of these 16 or 64 triad types, different characteristics associated with social network can be examined such as transitivity, cyclicity, mutuality (reciprocity) etc. Triadic methods have been used for studies in psychology, network evolution, business networks, neuroscience and security.
\\
\\
For a digraph with \(n-vertices\) there can be \(T = {^n\text{C}_3}\) triads. Naive algorithm for calculating triad census will take too much time - \BigO{n^3} time complexity. Faster algorithms for calculating triad census have been proposed. \citep*{Moody1998} proposed an adjacency-matrix based algorithm with quadratic complexity \BigO{n^2}. \citep*{Batagelj2001}  proposed algorithm with sub-quadratic time complexity \BigO{m\Delta} where \(m = \BigO{n.k(n)}\) is the number of arcs of the graph and \(\Delta\) is maximum degree of the graph. Multithreaded implementation of the sub-quadratic triad census algorithm was evaluated by \citep*{Chin2009}. There Multithreaded implementation is based on \citep*{Batagelj2001} subquadratic triad census algorithm. 
\\
\\
Now we briefly introduce with some notations and then explain the working of Subquadratic triad census algorithm. \(\{ \}\) denotes set notation, \(( )\) denotes ordered pair notation. Consider a strict digraph (no loops) \(G = [V, E]\) where \(V = \{1, 2... n\}\) is set of vertices and \(E \subseteq V x V \) the set of arcs (directed) i.e. \(E = \{(u, v), \, \exists u,v \in V \}\). Order of graph \(n = |V|\), size of graph \(m = | E |\). N is an array of neighbor lists indexed on vertex such that \(\forall u \in V\),  N(u) is the set of open neighborhood of vertex u i.e. \(N(u) = \{ v \in V | \{u, v\} \in E \}\). Note that N(u) contains all vertices v adjacent to u in undirected sense. 
\\
\\
The Subquadratic triad census algorithm(Figure~\ref{fig:triadcensus}) works by computing count of three triad types separately. It first counts all dyadic triads($T_{2}$) and connected triads($T_{3}$). Then it counts number of null triads $T_{1} = T - T_{1} - T_{2}$. Counting of the triads is basically based upon dyads in the digraph. The algorithm starts with initializing Census array to zero(lines 1-3). It then runs a for loop for each vertex of graph(lines 5-23). Within this loop, dyadic($T_{2}$) and connected triads($T_{3}$) are counted. 

\begin{figure}
\begin{flushleft}
\textbf{Function}: Subquadratic Triad Census Algorithm\\
\textbf{Input}: Graph \(G = [V, E]\) where V is set of vertices, E is array of edge lists and N is array of neighbor lists\\
\textbf{Output}: Census array with frequencies of isomorphic triadic types\\
\end{flushleft}
    \begin{algorithmic}[1]
	\For{$i = 1 \to 16$} 
	    \State Census[$i] \gets 0$
	\EndFor
	\\
	\For{ $u \in V$} 
		\For{ $v \in N[u]$}
			\If {$u$ \textless $v$}
			    \State $S \gets N(u) \cup N(v)  \setminus \{u,v\}$
				\If { $IsEdge(u,v) \wedge IsEdge(v,u)$ }
				    \State $TriadType\gets 3$
				\Else
	                \State $TriadType\gets 2$
				\EndIf
				\State $Census[TriadType] \gets Census[TriadType] + n - |S| - 2$
				\For{ $w \in S$ }
					\If{$v$ \textless $w \vee ( w$ \textless $v \wedge u$ \textless $w \wedge \neg IsNeighbour(u,w) )$}
		                \State $TriadType \gets TriadCode(u,v,w, )$
		                \State $Census[TriadType] \gets Census[TriadType] + 1$
		            \EndIf
				\EndFor
			\EndIf	
		\EndFor
	\EndFor
	\\
	\State $sum \gets 0$
	\For{$i = 2 \to 16$} 
	    \State $sum \gets sum + Census[i]$
	\EndFor
	\State $Census[1] \gets n*(n-1)*(n-2)/6 - sum$
	\end{algorithmic}
	\caption{Subquadratic Triad Census Algorithm}\label{fig:triadcensus}
\end{figure}

\begin{itemize}
\item \textbf{Counting number of dyadic triads($T_{2}$)}: a connected dyad (u, v) with u < v (line 7), contributes number of dyadic triads equal to all vertices of the graph except u and v themselves and except all vertices which are in open neighborhood of the connected dyad  i.e. \(n-|{u,v}|-|S|\) where \(S = N(u) \cup N(v) \setminus {u,v}\) is the set of vertices in open neighborhood of connected dyad (u,v)(see lines 8,14). Depending upon if the connected dyad (u, v) is asymmetric or mutual, all dyadic triads contributed by it are either of triad type 2-012 or 3-102 (line 9 to 13). The condition u < v (line 7) is necessary for canonical selection of a dyad. By canonical it means every non-null triad contributed by the connected dyad must be counted only once during different iterations of the algorithm. For example the connected dyad (1,2) is canonical but (2,1) is not. This is so because after counting the triads contributed by dyad (1,2), processing dyad (2,1) would lead to repetition of triad counting.

\item \textbf{Counting number of connected triads($T_{3}$)}: Each connected dyad (u,v) where u<v, also contributes number of connected triads equal to vertices in its open neighborhood set S(line 15-20). Again, all non-canonical selections must be eliminated. Three vertices forming a connected triad can be selected in six ways: (u,v,w), (u,w,v), (v,u,w), (v,w,u), (w,u,v) and (w,v,u). Line 7 already already made last four of these selections non-canonical by enforcing u<v condition. Line 16 determines which of the two remaining selections (u,v,w) and (u,w,v) is canonical. 

\begin{itemize}
\item Selection (u,v,w) with u<v< w  is always canonical. 
\item However if u < w < v, then this selection can be non-canonical only if u and w are neighbors because then the triad (u,v,w) was already counted in previous iteration of algorithm when dyad (u,w) was processed. 
Line 16 enforces condition to check if w forms part of a canonical triad: 

\begin{verbatim}
    v < w or ( w < v and u < w and !IsNeighbour(u,w) )
\end{verbatim}

\end{itemize}

$IsNeighbour(u,v)$ function checks if vertices u and v are neighbors in undirected sense. Line 17 finds isomorphic triad types using $TriadCode(u,v,w)$ function ( Figure~\ref{fig:TriadCode} ). This function first calculates triad code value between 0-63 corresponding to 64 non-isomorphic triad types. It returns this value + 1 if main algorithm calculates non-isomorphic triad census. Otherwise a mapping table $TriadTable$ maps the 64 non-isomorphic triad types to 16 isomorphic types and function then returns a value between 1 and 16. $IsEdge(u,v)$ function checks if a directed edge exists from u to v. Returns 1 if true, 0 otherwise. Finally the Census corresponding to triad type is incremented to count the connected triad (line 18).

\begin{figure}
\begin{flushleft}
\textbf{Function}: TriadCode\\
\textbf{Input}: vertices u, v, w\\
\textbf{Output}: isomorphic or non-isomorphic triad code
\end{flushleft}
\begin{algorithmic}[1]
\State $TriadCodeVal = IsEdge(u,v)$
\State $TriadCodeVal += 2 * IsEdge(v,u)$ 
\State $TriadCodeVal += 4 * IsEdge(u,w)$
\State $TriadCodeVal += 8 * IsEdge(w,u)$
\State $TriadCodeVal += 16 * IsEdge(v,w)$
\State $TriadCodeVal += 32 * IsEdge(w,v)$
\State $return ( IsIsomorphic ? TriadTable[TriadCodeVal]:TriadCodeVal ) + 1$
\end{algorithmic}
	\caption{Triad Code Algorithm}\label{fig:TriadCode}
\end{figure}

\item \textbf{Counting null triads($T_{3}$)}: Lines 24-27 stores sum of $T_{2}$ and $T_{3}$ in variable sum and subtracts this sum (line 28) from total count of all triads of the graph(line 28) to get count of null triads $T_{1}$
\end{itemize}

Time complexity of the of the above Subquadratic triad census algorithm is \BigO{m\bigtriangleup}. Exact complexity depends upon the sparsity of graph data set and the maximum degree of the graph. For small world networks with power law degree distribution that are sparse i.e. m is \BigO{n.k(n)} where $k(n)<< n$, and have small maximum degree i.e. $\bigtriangleup << n$, the algorithm complexity is linear - \BigO{n}. If maximum degree of graph is high i.e. $\bigtriangleup \backsim n$, then algorithm complexity is quadratic - \BigO{n^2}. For complete graphs, the time complexity becomes cubic - \BigO{n^3}

\section{Previous work}
\label{sec:triad-algo}
We now present details of previous work on multithreaded evaluation of Subquadratic census algorithm done by \citet{Chin2009}. We first discuss the details of the hardware software platform used by authors and then discuss their multithreaded implementation of triad census algorithm.
\\
\\
For evaluation, \citet{Chin2009} used Cray XMT supercomputer which consists of 4 Threadstorm(3.0) multithreaded VLIW processors, each supporting 128 hardware threads (streams). The platform had total shared system memory of 1 TB and included high-speed interconnect and network 3D-Torus topology. Like many multithreaded processor architectures, Cray XMT's are designed to tolerate memory access latencies through fine-grained multithreading. Out of many Multithreaded processor based systems in the market, Cray XMT's have been found to fit well the requirements of latency sensitive irregular graph algorithms and in the past many data intensive irregular algorithms \protect\footnote{\href{http://cass-mt.pnnl.gov/docs/XMTOverviewSC08BOF.pdf}{Source: PNNL, US}}  \protect\footnote{\href{http://user.cscs.ch/fileadmin/user_upload/customers/CSCS_Application_Data/Files/Presentations/Courses_Ws_2011/CRAY_XMT_Programming_Jun11/XMT_Tutorial_CSCS_1.pdf}{Source: CSCS, CH}} have performed well on this machine architecture. Light weight synchronization mechanisms along with high tolerance to memory latency make Cray XMT apt for such data intensive irregular applications.
\\
\\
The programming model of Cray XMT is essentially a distributed shared memory(shared address space) model. Programmer can create a multithreaded implementation in C/C++ using compiler pragmas and light weight synchronization constructs. The Cray parallelizing C/C++ cross compiler then compiles this code to generate low overhead light weight threads. The compiler also automatically parallelizes loops and nested loops whose range can be determined at compile time. It generates VLIW instructions that can hold up to three operations, comprising of control, arithmetic and memory operations. Special versions of load and store instruction are emitted by the compiler during parallelization.
\\
\\
Authors basically implemented and evaluated four versions of Subquadratic triad census algorithm on cray XMT. First, they implemented the original Subquadratic triad census algorithm with some variations. Second, they implement a distributed task queue based implementation of their modified subquadratic triad census algorithm. Each task is a canonical dyad and task queues are created sequentially. For synchronizing concurrent updates to census array, they used fast atomics. For storing graph data, both implementations used compact data structures(no details). For parallelization, they relied on ability of compiler to automatically parallelize loops(implicit parallelism) to generate multithreaded. Third and fourth implementations basically augment loops in their first and second implementations with \textit{loop future} compiler pragma to designate each iteration of the loop to be executed by a thread. For experimentation and performance evaluation, they used one real world graph data set and two tool generated random graph data sets. By iterating through phases of simulations--optimization (compiler directives, stream management, load balancing by interleaved loop iteration scheduling), they are able to obtain nearly linear speedups for most of their implementations on almost all data sets. In the end, they conclude that loop future versions fair better in terms of scaling and CPU utilization ( load balancing )

==> chapter-3/irregularoptimizations.tex <==
\chapter{Performance optimization's for irregular graph algorithms }
\label{chap:irregularoptimizations}
This chapter focuses mainly on discussing software and hardware techniques for performance optimization of irregular algorithms. In addition to presenting techniques specific for graph algorithms, it also discusses many generic performance optimization techniques. We first discuss irregularity problem in algorithms and some hardware-software techniques to tackle them. Next we explore efficient graph data structure representations and optimization's. Thereafter we present state of the art in cache aware algorithm and data structure design

\section{Irregularity in computation and communication}
\label{sec:irregcompcomm}
Many algorithmic problems in computer science exhibit a property called \emph{Irregularity} \citep{Yelick93datastructures} which makes it hard to obtain their efficient sequential and parallel implementations on multiprocessor systems. Irregularity is closely linked to the problem which the algorithm solves and also to the way it is represented. Some of the many problems that come with irregularity are unpredictability and lack of static patterns which makes it difficult to analyze such problems. Many authors have tried to identify properties of irregularity. Irregularity stems itself in many ways:

\begin{itemize}
\item \emph{Irregularity in flow control}: This is mostly the property of the algorithm itself and not necessarily of its representation/implementation. They result from presence of many conditional statements inside the program. Formulating alternative algorithmic solution to the problem may change the irregularity in its flow control. At a single thread level, hardware based speculative execution of instructions on both taken and not-taken side of the branch somehow improve the exploitable parallelism at instruction level. For Multi-threaded applications, hardware based techniques such as thread level speculation (TLS) techniques tries to address this it through coarse grained thread level parallelism. Software techniques includes predication, eliminating branches and loop unrolling.

\item \emph{Irregularity in data structure}: This is the property of representation and implementation of the data structures and its algorithms and generally not of the problem solution. Typically such programs create, insert, delete, update, and traverse data stored in array based data structures (data static or known priori) and dynamic pointer based data structures (for unknown/dynamic data). Examples of such data structures are sets, trees, graphs, unstructured grids. Most of the time linked data structures are used which involve pointer chasing. Depending upon the processor and memory architecture, the manner in which data is partitioned, mapped and traversed in the memory, execution of the algorithm for same or different data sets may result in different performance due to unpredictable cache effects, scheduling and load balancing issues. One way is to to try identify data access pattern and then map this data access pattern on the memory architecture. Still the data access patterns may differ from one data sets to another which makes it to difficult to stick to one particular methodology. 

\item \emph{Irregularity in communication}: Many programs contain data structures that can be partitioned to be operated by many similar threads as in data parallel applications or by different threads as in task parallel applications or a combination thereof. Most of the time threads of irregular applications are not completely decoupled from each other and have to communicate with each other or share some data and may also have to synchronize with other threads at some point. The thread communication typically is handled through either through shared memory(tightly coupled multiprocessors)  or through explicit message passing(loosely coupled multiprocessors). Depending upon the processor coupling, communication architecture (shared/distributed address-space/memory) and the data partition technique employed, the communication can take significant amount of the overall application execution time. How to generate good partitions of data associated with such irregular applications while keeping communication costs low and loads balanced across PE's is yet another topic of interest. Due to many non-deterministic events (interleaving of threads, cache misses etc.) and other issues(memory hierarchies, variance in bandwidth and latency), it becomes difficult to predict the overall communication cost.
\end{itemize}

So how exactly one should go about analyzing irregular applications for parallelization? In literature many approaches to study parallelism in irregular applications have been adopted. 

\begin{enumerate}
\item One approach is to provide frameworks to make them more regular as shown by authors in \citep{Panangaden2000}. They present a methodology of graph grammars for efficient partitioning of pointer based dynamic data structures used in graph applications. They specify notion of \emph{good partition} and \emph{partition-ability} and also provide formal definitions in terms of graph set theory. Graph grammars essentially specify how to modify a graph (axioms) locally based on presence of certain sub-graphs in it with some predefined properties called \emph{contexts}. The set of rules for carrying out these transformations are named \emph{productions} and sequence of graphs so generated using productions is called the \emph{language of the graph}. They further extend notion of graph grammars to parallel grammars which allow concurrent applications of many productions. In essence these graph grammars provide a model to make irregular data structures more analyzable or predictable by making them more regular thereby allowing user to derive good partitions.

\item Second approach of addressing irregularity and parallelism problems is by using a mix of algorithmic, data structure design and compiler techniques. Some of these techniques are architecture aware/oblivious algorithm and data structure design, static/dynamic thread scheduling and load balancing either done manually, or by operating system or by a run-time framework scheduler/load-balancer or in hardware. 

Compiler assisted techniques like \emph{Data Prefetching }hides memory load latency due to cache misses by inserting non-blocking load instructions. They have been successfully used for regular algorithms. Nevertheless they have also been studied on pointer based linked data structures. Authors in \citep{KarlStens2000} studied group prefetching of pointer nodes using auxiliary prefect array with overhead of memory. Similar studies \citep{ZhangTorrellas1995} have been done for share memory multiprocessors. Prefetching techniques have had limited success with irregular applications mainly due to obvious reasons: difficulty in predicting traversal-orders and prefetch distances, not enough work to hide memory latency, overhead of auxiliary data structures \& computations, strongly and multi-single strided profiling \citep{Srikant2002}, irregular control flows.

\item Another approach of approaching irregularity-parallelism problem is to treat regular algorithms as a special case of irregular algorithms as done by authors in \citep{PingaliKulkarni2009, PingaliDonald2011}. The authors in this study argue that instead of looking at data level parallelism in a mere simplistic way of \emph{same-operation performed on disjoint data sets}, it should be seen from a more data-centric point of view in terms of neighborhood and data structure elements. They propose that irregular computations have \emph{amorphous data parallelism}. Further they study patterns of this amorphous data level parallelism in number of irregular applications. In particular, they focused their study towards graph algorithms, and they introduce some intuitive abstractions inherent in graph algorithms: \emph{active element} - vertex or edge under a computation, \emph{activity} - a computation occurring over an active element or application of an operator, \emph{active region or neighborhood} - vertices and edges which are modified by the activity, \emph{morph} - operations which change structure of graph, \emph{local computations} - computations that change properties of vertices/edges, \emph{reader} - operations that retrieve property of a vertex or edge without changing graph structure. 

Another key graph algorithm characteristic that they identify is \emph{ordering} - one class of graph algorithms(\emph{unordered algorithms}) work correctly without any ordering semantics while other graph algorithms(\emph{ordered algorithms}) may impose some sort of order (total or partial ordering) in which vertices or edges are chosen or/and processed. For a set of active vertices and ordering constraints, they define amorphous data parallelism as parallelism that arises from simultaneous processing of active vertices subject to ordering constraints as well as any conflicts that may arise from overlap of active regions. Also ordering constraints and over-lapping of active regions may be statically visible at compile-time or dynamically generated at run-time. To exploit this parallelism when algorithm has ordering constraints, they propose to do speculative O-o-O (Out of order) execution of active computations in parallel but commit them in-order. They have proposed and devised a system-cum-tool called \emph{Galois system }and \emph{ParaMeter} \citep{Kulkarni2008} tool that can profile and assess an irregular algorithm and provide estimates of amorphous data level parallelism in it.

\item Finally hardware based techniques also try to address irregularity-parallelism problem in software independent manner. Irregular computations and data structures suffer from locality problems making them memory bound due to pointer-chasing. To address this problem requires memory latency hiding. Traditional hardware techniques which assist in memory latency-hiding are \emph{Prefetching, Cache memory hierarchy, TLB (Translation lookaside buffers) and Out-of-order execution}. These techniques continue to be used in present Multicore processors. More recently data-parallel intensive GPU architectures like NVIDIA Fermi are now integrating some of the ideas from GPP architectures(mainly cache hierarchies). Other hardware approaches to hide latency is implementing \emph{Hardware Multi-threading} in processor architectures. Hardware Multi-threading can hide memory latency arising from irregularity in memory access by exploiting high amount of thread level parallelism which can find enough work to hide memory latency.

\begin{itemize}
\item Scheduling another thread when a thread stalls on a cache miss (\emph{Block Multi-threading})
\item Scheduling many threads by interleaving their execution in each pipeline stage (\emph{Cooperative Multi-threading})
\item SMT(Intel Hyper-threading) architectures that combine Superscalar processing with hardware Multi-threading
\item Massively parallel architectures like GPGPU's which use a combination of fine-grained interleaved Multi-threading (at level of a warp) with a small cache hierarchy(NVIDIA Fermi)
\end{itemize}
\end{enumerate}
Thread level speculation is yet another technique. For more information on Hardware Multithreading and other related concepts, please see the \textbf{Appendix - B on Processor Architecture and micro-architecture}. In later sections, we will employ many of the above outlined ideas to tackle irregularity in Triad Census algorithm.

\section{Graph data structures}
\label{sec:graphds}
One major area which impacts performance of graph algorithms is the graph data structure that stores graph data and allows for traversal and manipulation of the graph. Which graph data structure is good for the graph algorithm depends upon many factors like graph size, dynamic/static graph algorithm, graph density, hardware resources, algorithm specific requirements (data partition-ability, fast insertions, deletions, traversal etc.). %All discussions on graphs from here on will use the terminology from \textbf{Graph theory and algorithms section }in \textbf{Appendix - C}.
\\
\\
In graph algorithmic theory, there are mainly two representations that can be used for representing graphs: \emph{Adjacency Matrix} and \emph{Adjacency Lists}. For a graph \(G = [V, E]\) with $n$ vertices and $m$ edges(undirected graphs) or arcs(directed graphs), an adjacency matrix uses an $n x n$ matrix to represent list of edges or arcs. Each location $[i,j]$ of the matrix stores a 1 or edge weight $w_{ij}$ if there is an edge(or arc) between(from) vertex $v_{i}$ and(to) $v_{j}$ otherwise a 0 is stored.
\\
\\
\emph{Adjacency Matrix} representation(Table~\ref{tab:adjmatrix}) is good for dense graphs and small order graphs (dense/sparse) but uses lot of space \BigO{n^2}. Its nice property is that elements of the data structure are accessed in contiguous fashion and so is cache and prefetch friendly. For sparse graphs, adjacency matrix wastes lot of space as there will be lot of zeros and instead adjacency list is preferred which uses space of order \BigO{|V|+|E|}.
\\
\\
\emph{Adjacency List }representation( Figure~\ref{fig:adjlist} ) of a graph \(G = [V, E]\) is a one dimensional array Adj of size $N = |V|$. For a vertex $v$ of graph $G$, $Adj[v]$ stores pointer to list of vertices adjacent with $v$. For weighted and digraphs, each adjacent list has an additional field to hold weight for that edge. Main problem with adjacency list representation is that finding whether an edge $(u, v)$ is present in graph requires traversal of adjacency list of $Adj[u]$. As lists are normally implemented as linked lists, they have further overhead of cache unfriendly design as they have poor spatial locality and cause cache miss for every node access in worst case - \BigO{n}. Even in the best case, when the nodes are allocated consecutively in order, because linked list nodes are larger, it can require several times more cache misses to traverse the list. To overcome this problem there are few approaches:

\begin{figure}	
	\includegraphics[scale=0.6]{chapter-3/images/dg}
	\caption{Directed graph}\label{fig:digraph}
\end{figure}

\begin{table}
  \centering
  \caption{Adjacency matrix representation of a graph}
  \begin{tabular}{ *{8}{c}}
     & V0 & V1 & V2 & V3 & V4 & V5 & V6\\
  V0 & 0  & 1  & 1  & 1  & 0  & 0  & 0\\		     
  V1 & 0  & 0  & 0  & 0  & 0  & 0  & 0\\
  V2 & 0  & 0  & 0  & 0  & 0  & 0  & 0\\
  V3 & 0  & 0  & 0  & 0  & 1  & 1  & 0\\
  V4 & 0  & 0  & 0  & 0  & 1  & 0  & 0\\
  V5 & 0  & 0  & 0  & 1  & 0  & 0  & 0\\
  V6 & 0  & 0  & 0  & 0  & 0  & 0  & 0\\
  \end{tabular}
  \label{tab:adjmatrix}   
\end{table}

\begin{figure}
		\centering
		\includegraphics[scale=0.6]{chapter-3/images/adjacencylist}
		\caption{Adjacency list representation of a digraph}\label{fig:adjlist}
\end{figure}

\begin{enumerate}
\item \emph{Cache blocked or unrolled linked lists} \protect\footnote{\href{http://www.wikipedia.com}{http://www.wikipedia.com}}: An unrolled or cache blocked linked list stores more than 1 element in each node of linked list. The elements inside the node are usually stored as array which provide good spatial locality. It is thus simply linked list of arrays(Figure~\ref{fig:unrolledlist}). Only one additional meta-data information is stored in each node of unrolled linked list which is a variable that stores number of valid elements stored in the array. As some elements of array may remain unfilled, the value of this variable is less than array length. Further, maximum number of elements stored in element array of node and alignment of node can be chosen carefully to match cache line size of the processor. This has two major advantages. First, as number of elements inside the node is more than one, the amount of memory space overhead(link pointers, alignment, other meta-data etc.) of a normal linked list is amortized due to blocking and thus it reduces memory space requirements. Secondly as each node contains an array of elements whose size is chosen according to cache line size, the spatial locality improves and as adjacency list is usually traversed from one element to next, this reduces number of cache misses. Further , accuracy of compiler inserted or hardware assisted prefetching increases.

\begin{verbatim}
      n = Elements inserted
      B = Cache line size in terms of number of elements
      N = blocking size in terms of number of elements
\end{verbatim}

Cache misses on traversing the list of $n$ elements in
\begin{itemize}
\item Array - \BigO{n/B}
\item Linked list - \BigO{n}
\item Unrolled linked list - \BigO{(n/N+1)(N/B)} [Note traversing elements in each node require \BigO{N/B} cache misses. Further assumption is all nodes are full]
\end{itemize}

As can be seen, the number of cache misses in unrolled linked list is close to optimal cache misses in arrays i.e. \BigO{n/B}. A blocked or unrolled linked list thus combines spatial locality benefits of arrays with quick insertion and dynamically re-sizing capabilities of a linked list. Only disadvantage of this approach for adjacency list representation of Graphs is that, if there is too much divergence in degrees of different vertices of the input graph, then there could be wastage of memory in linked list for nodes with very low degrees as the node array will be partially filled. If graph has large number of such low degree nodes, overall memory wastage will increase. Also, there is higher programming effort involving changes to data structures and also algorithms(insert/delete elements, traversal) which become more complicated. Portability of such implementations across another processor architecture may further require tuning.

\begin{figure}
	\centering
	\includegraphics[scale=0.5]{chapter-3/images/unrolled}
	\caption{Normal linked list and Unrolled(blocked) list}\label{fig:unrolledlist}
\end{figure}

\item \emph{Adjacency array representation}\citep{Mehlhorn.Sanders2008}: This representation stores combined adjacency information of all vertices in an array and uses an auxiliary array to remember starting position of adjacency array of each vertex. The small adjacency arrays for all vertices can be concatenated into a single edge array $E$. An additional array $V$ stores the starting index positions of the individual adjacency arrays in $E$, i.e., for any vertex $v$, $V[v]$ is the index in $E$ of the first edge out of $v$. This representation( Figure~\ref{fig:adjarray} ) is same as the CRS(Compressed Row Storage) format used for representing sparse matrices
\protect\footnote{\href{http://software.intel.com/sites/products/documentation/hpc/mkl/mklman/GUID-9FCEB1C4-670D-4738-81D2-F378013412B0.htm}{Intel MKL CRS Format}}. In CRS terminology, array $V$ is called \emph{Row index array} and array $E$ is called \emph{Column Array}. \emph{Value array} of CRS format normally would represent weights or any other edge property and is thus optional.

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{chapter-3/images/adjacencyarray}
    \caption{Adjacency array representation of a digraph. Top array $V$ is the row index array of length $Size(G) + 1$. Lower array $E$ is the column or edge array of length $Order(G)$}\label{fig:adjarray}
\end{figure}

The edges out of any vertex v are then easily accessible as $E[V[v]] \ldots E[V[v + 1] − 1]$;
Normally a dummy entry $V[n + 1]$ with $V[n + 1] = m + 1$ is added to ensure that this also holds true for vertex $n$. Figure~\ref{fig:adjarray} shows an example. The memory consumption for storing a directed graph using adjacency arrays is $n + m + Theta(1)$ words.

\end{enumerate}

\subsection{Related Work}
\label{subsec:relatedwork}
Various graph data structure representations have been used in implementing graph algorithms on high performance processor architectures. \citet{Park.etal2004} studied cache-aware and cache-oblivious based data structure design techniques for various sequential graph algorithms. They demonstrate good execution speedups for Dijkstra's single-source shortest path algorithm and Prim's minimum spanning tree using cache-aware adjacency array representations. Further, they obtain significant speedups using cache-oblivious recursive implementation for Floyd-Warshall algorithm. They also combine adjacency array based approach and cache-oblivious approach and apply it to matching algorithm for bipartitie graphs.
\\
\\
\citet{Madduri2009c} used variety of representations for dynamic parallel graph algorithms involving run-time parallel insertion/deletions in large scale graphs of small-world networks on on Ultra Sparc T2 and IBM p5 570 SMP. They implement adjacency lists as \emph{Dynamic Arrays} - resizable adjacency arrays - as dynamic graph algorithms require structural updates during run-time. Such a structure allows for fast insertions and deletions for low degree vertices. To handle problems of frequent re-sizing of dynamic arrays, they do a large memory allocation initially. When re-sizing is required, they double the array size, essentially making a trade-off between number of re-sizes and memory footprint. Another data structure that they experiment for adjacency representation is \emph{treap} which allows faster deletions than dynamic arrays. The re-sizing strategy used for treaps is similar to dynamic arrays. Finally they make a hybrid adjacency representation which uses dynamic arrays for low degree vertices and treap for high degree vertices.
\\
\\
A number of graph representations have been studied on Manycore Processor Architectures like GPGPU's. \citet{Harish2007} implemented and evaluated number of graph algorithms using \emph{Adjacency Array and Adjacency Matrix} based representations namely breadth first search, st-connectivity, single-source shortest path, all-pairs shortest path, minimum spanning tree, and maximum flow algorithms. \emph{Edge list}representations is used in \citep{Pradesh2010} for implementing graph connectivity algorithms. Authors in \citep{Dehne2010} used optimized linked list representation for irregular graph algorithms like list ranking and connected components. They use arrays and sub-lists to improve performance bottlenecks associated with obtaining good performance on GPU's. Further they make some comparisons of speedups obtained on SMP's and GPU's.

\section{Cache aware optimization and data structure design}
\label{sec:cacheoptim}
In many traditional and modern processor architectures, there exists \emph{Multilevel Memory Hierarchy }where each level act as a cache for next. A typical hierarchy consists of registers, level 1 cache, level 2 cache, level 3 cache, main memory(DRAM), and disk. The underlying importance of this hierarchy is that as the memory level gets farther from the CPU, it becomes larger in size and slower(high latency). Typically registers and level 1 caches are the fastest when compared to other memory levels. The difference in memory access time increases dramatically from level caches to DRAM.
\\
\\
An instruction which needs to access data from a memory address, can execute only if the required data is present or brought in closest cache level. Instruction thus waits for the data if its in farther memory levels. A consequence of this is that in order to obtain high algorithmic performance, it is important to make sure the accessed data is held by closest memory level. This problem of making sure that accessed data always resides in closest level (atleast in some level cache) - i.e. memory access latency is low - is non-trivial to solve, depends upon many factors and requires careful algorithmic and architecture specific design optimization's.
\\
\\
Optimizations which are specifically applied to keep data in on-chip level caches are called \emph{Cache Optimizations}. Cache optimizations can be both \emph{architecture aware} and \emph{architecture oblivious}. If Cache optimization's require detailed knowledge of underlying cache hierarchy(levels, block sizes, alignment) then it is called \emph{Cache Aware}, otherwise \emph{Cache oblivious} \citep{Demaine2002, Kumar2003, Arge2005}
\\
\\
Many optimizations exist in literature \citep{Srikant2002, Drepper2007, Garg.Sharapov2001} that can be used to address the memory latency problems. They basically try to do the following:
\begin{itemize}
\item Reduce cache misses(cold, capacity and conflict)
\item Reduce latency to serve a cache miss
\end{itemize}

\begin{table}[!hb]
  \centering
  \caption{Memory hierarchy optimization summary}
  \begin{tabular}{ | p{6cm} | p{7cm} | }
  \hline
  \textbf{Optimization} & \textbf{Performance improvement}\\ \hline
  Cache blocking(linked lists) & Fewer cold misses\\ \hline
  Cache blocking(arrays) & Fewer capacity misses\\ \hline
  Sorting linked lists in sequential order of node addresses & Fewer cold misses, better prefetching, amortized average load latency\\ \hline
  Prefetching using auxiliary structures(linked lists) & Reduces cold misses, aids prefetching\\ \hline
  Reduce cache pollution and pack caches with useful data & Better cache utilization and reduced bandwidth wastage\\ \hline
  Cache aligned data structures & Lower cache footprint, halves cache misses due to misalignment\\ \hline
  Keep hot fields together and access in layout order & Higher cache utilization, reduced capacity misses due to lower cache footprint, more efficient prefetching\\ \hline
  Loop interchange & Fewer conflict misses ( cache thrashing \footnotemark )\\ \hline
  Loop fusion & Fewer conflict misses\\ \hline
  Loop fission & Fewer conflict and capacity misses\\ \hline
  Loop unrolling & Increases ILP, lowers loop overhead\\
  \hline
  \end{tabular}
  \label{tab:memoryoptimizations}   
\end{table}

\footnotetext{\emph{Cache thrashing} is a term used for conflict and/or capacity misses which occur due to time multiplexed sharing or contention of same cache line and/or due to big size of working data. A related concept with cache thrashing is \emph{False Sharing} when two different and unrelated memory locations accessed(written by at least one thread) by different threads tend to fall on the same cache line. This leads to contention of the same cache line causing cache thrashing. This mainly happens when two different memory address locations map to the same cache line i.e. they have same value for (mem\_address\_loc \% (cache\_sz/cache\_assoc)). Types of data which is susceptible to false sharing can be statically allocated (e.g., globals, statics), heap allocated, automatics and thread-locals (if pointers/references handed out).}

Most of the techniques rely on code-restructuring, data-layout and data access optimizations to tackle irregularities in memory access. Another aspect of improving locality of data layout and access is that TLB misses would also decrease because with good locality most data will be accessed from locations in the same page. We have already discussed prefetching and cache-blocking. This section will discuss other techniques that can be used with algorithms and data structures used in graph algorithms. Table~\ref{tab:memoryoptimizations} shows the summary of these memory optimizations.
\\
\\
As described in earlier sections, for Sparse Graphs, Adjacency list is the defacto representation. There are mainly two ways to design and implement an adjacency list: \emph{Adjacency array} and \emph{Cache blocked linked lists}. Adjacency array based representation are static and thus have many limitations due to which it cannot be used in many practical graph algorithm implementations particularly when graph data sets to be processed are dynamic in nature as in online algorithms. As a result many graph algorithm implementations eventually need to use linked lists based representations. As the linked list data structure is central to adjacency list representation, it is important to make it cache friendly. In literature there exists many optimization and data structure design techniques ( Table~\ref{tab:memoryoptimizations} ) that can be applied to linked lists to effectively leverage cache hierarchy of the processor:

\begin{enumerate}
\item \emph{Cache blocking the linked list}: Its basics have already been discussed before. There is plenty of material available on how to implement blocked linked lists and tune block sizes \citep{Frias2010}. Intel \protect\footnote{\href{http://software.intel.com/en-us/articles/cache-block-size-on-processors-that-support-hyper-threading-technology}{http://software.intel.com/en-us/articles/cache-block-size-on-processors-that-support-hyper-threading-technology}} suggests using a block size which is 50\% to 75\% of cache line size.

\item \emph{Sort the linked list layout}( \citep{Madduri2009d} ): Nodes of a linked list are normally allocated in non-contiguous memory locations. In the worst case this causes cache miss on every load operation. By sorting the elements of the linked list in a sequential memory address order, many cache misses can be avoided as there is a possibility that many nodes may occupy the same cache line. Also, as PE's in many Multicore processors still has the ability to execute instructions Out-of order, the processor can now better overlap multiple load operations for successive node accesses by issuing memory access requests in advance. This can somewhat hide memory latency by having many load operations in-flight. Speculative prefetches will also become more accurate.

\item \emph{Auxiliary data structure to improve Prefetching}\citep{AMD2008}: Another technique is to create a separate history array that stores addresses of linked list nodes in sequential order. During subsequent traverse of the linked list, this history array is traversed concurrently by the code and is used to prefetch the linked list elements that will be needed in the near future. The purpose of doing this is to have data already prefetched in L1 cache level from next address location in history array before it's needed. By doing a non-temporal prefetch it will not be subsequently evicted to L2 cache level.

\lstset{language=C}
\begin{lstlisting}
// Source: AMD
void build_history_array(linky* list, linky** history_array) 
{
  while(list) 
  {
    *(history_array++) = list;
    list = list->next;
  }
}

linky* traverse_list_with_history (linky* list, linky** history_array, int n) 
{
  while(list) 
  {
    // Non-temporal prefetch
    _mm_prefetch((char*) *(history_array + n), _MM_HINT_NT);
    history_array++;
    list = list->next;
  }
  return list;
}
\end{lstlisting}
This technique works well when node size is small and linked list structure is not updated frequently.

\item \emph{Avoid wasting cache space}: Choose member data type according to range of actual data values and try to utilize all locations in each cache line for useful data. Avoid using large data types when a smaller type can be sufficient. As a result more data can be read or written per cache line access.

\item \emph{Reduce cache pollution}\citep{Park.etal2004}: \emph{Cache pollution} is related to repetition of cold misses for same memory location. As long as relevant data is there in the cache, use it there and then only as much as possible before it gets replaced. This also reduces the bandwidth overhead due to reduced data transfer round trips between memory and processor

\item \emph{Cache aligned data structures}(\citep{Fry2008}): On a cache miss, when a cache line is moved from main memory to last level cache(LLC) or between cache levels. It is brought as a cache line aligned to boundary of cache line size. If access to a memory location or a group of memory locations(example a structure access) is not cache aligned, extra cache lines need to be fetched to load all data. This will result in one extra cache line fetch which further exacerbates overall access latency. Thus unaligned memory access can be twice slower than aligned memory access. Another associated problem could be increase in conflict misses for the extra cache line fetched. To avoid this, pack data structures with members such that they fit evenly on cache line boundaries.
\\
\\
Memory alignment of an object instance of a data structure and members within object in-stance is determined by the memory alignment of its largest member. This is almost always smaller than the cache line size. This means even if the members of a structure are lined up to fit into the same cache line an allocated object might not have an alignment matching the cache line size. Only way to deal with it is to force cache aligned memory allocation. Below are examples of some constructs that force memory alignment:

\begin{itemize}
\item For static objects, use attribute(for gcc)
\begin{lstlisting}
type variable __attribute((aligned(line_sz)));
struct strtype 
{
..members..
} __attribute((aligned(line_sz)));
\end{lstlisting}
\item For dynamic allocation \emph{posix\_memalign} instead of \emph{malloc} can be used to request higher alignment
\item Programmatically forcing can also be done
\end{itemize}

Problem with enforcing memory alignment is that it can cause memory fragmentation and higher memory consumption because of padding bytes. To reduce padding bytes, manually reordering data structure members in ascending/descending order or compiler directed packing can reduce padding due to misaligned members of data structure. SSE2 instructions on x86 CPU's do require the data to be 128-bit (16-byte) aligned and there can be substantial performance advantages from using aligned data on these architectures.

\item \emph{Hot fields should be placed together and accessed in order of layout }\citep{Srikant2002, Fry2008}: Arrange layout of member items of a structure in order of frequency of access and also order in which they will be accessed. This will divide the memory layout of structure in groups of hot fields(higher access frequency) and cold fields(rarely accessed). As a result, group temporal/spatial re-usability increases as clubbed items are more likely to be accessed together. With this, the chances that clubbed items occupy the same cache line increases. Also by accessing the items within hot field in order of their layout, the prefetch mechanism can work more accurately. Further, techniques like structure splitting can be used to divide big data structures that occupy cache lines unevenly into small data structures that more evenly fit cache lines.

\item \emph{Loop optimizations}\citep{Srikant2002}: Many loop specific optimizations can be used for structures other than linked lists. \emph{Loop-blocking or strip-mining }makes tiles or blocks of data size related to cache line size and basically reduce capacity misses. \emph{Loop interchange} improves spatial locality by interchanging nested loops to traverse data in continuous dimension(innermost array dimension in C, outer-most array dimension in FORTRAN). \emph{Loop fusion} amortizes cache misses by fusing two independent loops with compatible indexes. \emph{Loop fission} reduces splits a loop into many loops to reduce the memory footprint of loop iteration thereby reducing capacity misses. \emph{Loop unrolling} is a technique that reduces loop overheads, increases ILP, reduces control flow and improves cache utilization by data reuse. It is effective when loops enclose low to moderate amount of computation and contains very few function calls.
\end{enumerate}

\section{Reducing Branches and improving flow control}
\label{sec:branchoptim}
All programming constructs like if-else, goto, switch, while/for loops, function calls etc. on compilation generate branch instructions. Instruction stream containing high percentage of branch instructions cause control hazards(irregular control flow), resulting in processor pipeline stalls and thus can deteriorate performance. For irregular algorithms, many branches tend to be data dependent and thus branch predictors in Multicore processors have hard time in correctly predicting these branches. On GPU processors, presence of unpredictable data dependent branches can significantly lower the performance if different threads tend to follow different branch paths ( called as \emph{warp divergence} ). 
\\
\\ 
In other words, processors work best when control flow is sequential. Consequently, optimizing branches should be one of the optimization priorities and can yield good performance improvements. Some of the techniques to optimize branches are: 

\begin{itemize}
\item \textbf{Eliminate branches}: The simplest way to optimize branches is to try to eliminate unnecessary branches. Most of the time, this requires analysis at algorithmic and code level. This is the simplest and least effort branch optimization which can reduce irregular control flow and yield good performance improvements. 
\item \textbf{Loop unrolling} reduces number of loop iterations and consequently reduces the branch penalties. Loops with static or predictable iteration bounds can be easily unrolled either by the compiler or explicitly by programmer. For loops whose iteration range at compile time is not predictable or unknown, the programmer can explicitly unroll the loops with extra programming effort.
\item \textbf{Function inlining} is another branch optimization technique which is also normally done by the compiler but the programmer can also control it programatically. When a function is \emph{inlined}, all calls to this function in the entire program are replaced with the actual function code by the compiler. For functions with small code size and which are called very frequently, function inlining makes sense and can yield good performance improvements. Note that compilers may ignore the inlining of a function.
\item \textbf{Predication} is a branch optimization technique which is normally employed by compilers. When a branch is predicated by the compiler, all instructions in different branch paths are predicated with the branch condition. All the predicated instructions are executed by the processor irrespective of the branch condition, however only those instructions for which the predicate condition is true are committed. Compiler based predication thus requires support at ISA level of the processor. Although compilers are able to optimize many branches with predictable paths but data dependent branches poses significant challenges for compiler. For such data dependent branches, the user can programatically implement predication.
\end{itemize}
